Neural Image Compression: Generalization, Robustness, and Spectral Biases

Recent advances in neural image compression (NIC) have produced models that are starting to outperform classic codecs. While this has led to growing excitement about using NIC in real-world applications, the successful adoption of any machine learning system in the wild requires it to generalize (and be robust) to unseen distribution shifts at deployment. Unfortunately, current research lacks comprehensive datasets and informative tools to evaluate and understand NIC performance in real-world settings. To bridge this crucial gap, first, this paper presents a comprehensive benchmark suite to evaluate the out-of-distribution (OOD) performance of image compression methods. Specifically, we provide CLIC-C and Kodak-C by introducing 15 corruptions to the popular CLIC and Kodak benchmarks. Next, we propose spectrally-inspired inspection tools to gain deeper insight into errors introduced by image compression methods as well as their OOD performance. We then carry out a detailed performance comparison of several classic codecs and NIC variants, revealing intriguing findings that challenge our current understanding of the strengths and limitations of NIC. Finally, we corroborate our empirical findings with theoretical analysis, providing an in-depth view of the OOD performance of NIC and its dependence on the spectral properties of the data. Our benchmarks, spectral inspection tools, and findings provide a crucial bridge to the real-world adoption of NIC. We hope that our work will propel future efforts in designing robust and generalizable NIC methods. Code and data will be made available at https://github.com/klieberman/ood_nic.

==> sec_image_compression.tex <==
\section{Image compression methods}
\label{sec:img_compression}
%\BK{This should be deferred to the appendix given this section is already short. }

Here we provide details on the NIC methods considered in our analysis. 

%\subsection{NIC and JPEG2000}
%\label{subsec:nic-jpeg}
\noindent{\textbf{Fixed-Rate NIC.}} We use the hyperprior model \(\mathcal{C}\) proposed by Ball\'e \etal as our base NIC model \cite{balle2018variational}. 
This model consists of an autoencoder that encodes the image $X$ to latent space $Y$, quantizes $Y$ to $\hat{Y}$ and finally synthesizes $\mathcal{C}(X)$ from $\hat{Y}$. 
In practice, the quantized latent vector $\hat{Y}$ is entropy encoded before transmission.
Each of the components of the autoencoder has three convolutional layers, with the number of channels controlled by parameters $N$ and $M$. 
Generalized divisive normalization (GDN) and inverse-GDNs are used as the non-linear activation functions in the auto-encoder. 
GDNs implement local divisive normalization and have been shown to be particularly effective in image compression tasks \cite{Balle2015-ha, balle2017endtoend}.
The model also has a hyperprior autoencoder with the exact same architecture as the other autoencoder, except with ReLU non-linearities. 
%\cwg{although doesn't the hyper prior model use different non-linearities?}\KL{yes, good point}.
This encodes the prior on the entropy coding model and has been shown to improve performance. 
We based our implementation off of the one from \cite{begaint2020compressai}.

% \begin{enumerate}
%     \item Dense fixed-rate
%     \item Pruned fixed-rate
%     \item Dense variable-rate
%     \item Pruned variable-rate 
%     \item JPEG2000
% \end{enumerate}
% Although their performance on rate-distortion curves is quite promising, NIC models are still known to be computationally expensive. These models have several million learned parameters. Training requires thousands of images and a few days of computation on specialized GPUs. It is possible for inference to be done without a GPU, but this is very slow. Additionally, despite their size, these models usually only work at one compression rate or a small range of compression rates \cite{Minnen_2018, Yang_2021_CVPR}. In the past, if variable-rate compression is desired, several models must be trained and stored separately. This, on top of the model's large size to begin with, makes variable-rate NIC infeasible for use on edge devices. In this section, we demonstrate that NIC models themselves can be approximated (\ie, we can compress the compressor) and we propose a single sparse model which can be used over a wide range of compression rates.

%\subsection{Variable-Rate NIC}
\noindent{\textbf{Variable-Rate NIC.}}
For our variable-rate NIC we implemented a model proposed by \citet{Dosovitskiy2020You}. 
This model uses Loss Conditional Training (LCT) to train a variable-rate NIC 
based off the hyperprior model outlined in the previous paragraph.
%based off of the model described in Section~\ref{subsec:nic-jpeg}. 
The model is trained over a continuous range of compression rates, optimizing the rate-distortion tradeoff at each. 
Once trained, this model can be adaptively used at any compression rate in the range, which makes it even more flexible than a discrete set of fixed-rate models. 
In order to condition the compression rate via LCT, all convolutional layers in the model are augmented with Feature-wise Linear Modulation (FiLM) layers \cite{Perez_2018_film}. 
In this case, these are small neural networks that take a conditioning parameter $\lambda$ as input and output a $\boldsymbol{\mu}$ and $\boldsymbol{\sigma}$ used to modulate the activations channel-wise based on the value of $\lambda$. 
More details on FiLM layers are provided in Appendix~\ref{app:film}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Specifically, suppose a layer in the CNN has activations $\boldsymbol{f}$ of size $W \times H \times C$, then $\boldsymbol{\mu}$ and $\boldsymbol{\sigma}$ are both vectors of size $C$ and the augmented activations $$\boldsymbol{\Tilde{f}} = \boldsymbol{\sigma} \mathbf{f} + \boldsymbol{\mu}.$$
Figure \ref{fig:film_diagram} shows a diagram of FiLM layers being applied to a small example network. Normally, without FiLM layers, the equation to calculate the features maps is
\begin{align}
    \mathbf{x}^{(1)} = \rho(W^{(1)}\mathbf{x}^{(0)} + \mathbf{b}^{(1)}),
\end{align}
where $\rho$ is the activation function (\eg, ReLU). However, with FiLM layers, the weighted sum is first subject to augmentation with $\mu$ and $\sigma$. Thus, the new calculation is
\begin{align}\mathbf{x}^{(1)} = \rho(\boldsymbol{\sigma}^{(1)}(W^{(1)}\mathbf{x}^{(0)} + \mathbf{b}^{(1)})) + \boldsymbol{\mu}^{(1)}).
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%During training, a random $\lambda$ is drawn with each mini-batch and used in two ways: 1) as input to the FiLM layers to modulate the feature maps and 2) in the mini-batch's loss function. During inference, the model takes as input a desired compression rate $\lambda$ along with the input image. Notably, LCT and FiLM layers only affect the values of the activations (\ie, feature maps), but not the \textit{weights} on the convolutional layers or activation functions. This is an essential observation for applying pruning to the network. 

\iffalse
\subsection{Pruning NIC Models}
%A limitation of using NIC in the wild is the size of the NIC models. 
%These models require several million learned weights and efficient inference requires specialized GPUs. 
%This limits the possibility of using NIC on an edge device, like a drone or a cell phone. 
%In this section, we demonstrate that NIC models themselves can be approximated (\ie, we can compress the compressor) and we propose a sparse versions of both fixed-rate and variable-rate NIC models.
%
% However, there are many situations in which one would want to perform image compression on an edge device. 
%This limits the effectiveness of NICs in the wild because they can not be used on edge devices.
% NIC models are known to be computationally expensive, requiring several million learned parameters and efficient inference on these models requires specialized GPUs. 
%
To prune our %fixed- and variable-rate 
NIC models, we propose gradual magnitude pruning (GMP) \cite{zhu18_gmp} based approach which has been demonstrated to effectively sparsify DNNs. 
%At a high level, 
GMP gradually prunes DNN weights based on their magnitude over a fixed number of epochs then continues to train, or fine-tune, the remaining sparse network after the target sparsity is reached.
%The pruning can be done layer-wise (\ie, the mask must be updated such that each layer has the target sparsity) or globally (\ie, the overall network must have the target sparsity, but the sparsities can differ between layers). 
%We utilized global pruning which has been demonstrated to produce more performant sparse models.
We utilized global GMP when training our pruned NIC models.
More details of the GMP algorithm are provided in Appendix~\ref{app:gmp}.
\fi

